Fundamental Tradeoffs in Learning with Prior Information

We seek to understand fundamental tradeoffs between the accuracy of prior information that a learner has on a given problem and its learning performance. We introduce the notion of prioritized risk, which differs from traditional notions of minimax and Bayes risk by allowing us to study such fundamental tradeoffs in settings where reality does not necessarily conform to the learner's prior. We present a general reduction-based approach for extending classical minimax lower-bound techniques in order to lower bound the prioritized risk for statistical estimation problems. We also introduce a novel generalization of Fano's inequality (which may be of independent interest) for lower bounding the prioritized risk in more general settings involving unbounded losses. We illustrate the ability of our framework to provide insights into tradeoffs between prior information and learning performance for problems in estimation, regression, and reinforcement learning.

==> sections/things-to-do.tex <==
\section{Things to think about}

\begin{itemize}
\item Experiments on generalization in RL/robotics. Can we construct examples that are challenging? In addition, can we implement a robustness argument using a hard learning problem? 
\item Numerical experiments with Occam’s razor/PAC-Bayes; maybe try on the example from Shay’s paper (or just the Bernoulli example).
\item Potentially study if PAC-Bayes is tight for prioritized risk (probably not). I could take a look at Theorem 4.4 in \href{https://www.cs.cmu.edu/~jcl/papers/tutorial/tutorial.pdf}{https://www.cs.cmu.edu/~jcl/papers/tutorial/tutorial.pdf}. If not, can we come up with something tight?
\end{itemize}
